Local and Global Graph Modeling with Edge-weighted Graph Attention Network for Handwritten Mathematical Expression Recognition

In this paper, we present a novel approach to Handwritten Mathematical Expression Recognition (HMER) by leveraging graph-based modeling techniques. We introduce an End-to-end model with an Edge-weighted Graph Attention Mechanism (EGAT), designed to perform simultaneous node and edge classification. This model effectively integrates node and edge features, facilitating the prediction of symbol classes and their relationships within mathematical expressions. Additionally, we propose a stroke-level Graph Modeling method for both local (LGM) and global (GGM) information, which applies an end-to-end model to Online HMER tasks, transforming the recognition problem into node and edge classification tasks in graph structure. By capturing both local and global graph features, our method ensures comprehensive understanding of the expression structure. Through the combination of these components, our system demonstrates superior performance in symbol detection, relation classification, and expression-level recognition.

==> 2172.tex <==

	\tikzset{stroke/.style={black, line width=0.1mm}}

	\begin{tikzpicture}
\draw [stroke] (0.0,0.83) -- (0.0,0.84) -- (0.0,0.84) -- (0.01,0.84) -- (0.01,0.85) -- (0.02,0.85) -- (0.03,0.86) -- (0.05,0.88) -- (0.06,0.89) -- (0.09,0.9) -- (0.11,0.92) -- (0.13,0.93) -- (0.15,0.95) -- (0.17,0.96) -- (0.2,0.97) -- (0.22,0.97) -- (0.25,0.97) -- (0.27,0.97) -- (0.29,0.96) -- (0.31,0.94) -- (0.33,0.92) -- (0.33,0.9) -- (0.34,0.88) -- (0.34,0.85) -- (0.33,0.81) -- (0.33,0.77) -- (0.31,0.73) -- (0.3,0.69) -- (0.28,0.65) -- (0.26,0.62) -- (0.25,0.58) -- (0.23,0.56) -- (0.21,0.54) -- (0.2,0.52) -- (0.19,0.52) -- (0.18,0.53) -- (0.18,0.54) -- (0.18,0.56) ;
\draw [stroke] (0.61,0.9) -- (0.61,0.91) -- (0.62,0.91) -- (0.62,0.91) -- (0.61,0.92) -- (0.61,0.92) -- (0.61,0.92) -- (0.61,0.92) -- (0.6,0.93) -- (0.6,0.93) -- (0.6,0.93) -- (0.59,0.93) -- (0.58,0.93) -- (0.57,0.92) -- (0.55,0.91) -- (0.53,0.89) -- (0.51,0.87) -- (0.49,0.84) -- (0.48,0.81) -- (0.46,0.78) -- (0.45,0.75) -- (0.45,0.73) -- (0.45,0.71) -- (0.45,0.69) -- (0.46,0.68) -- (0.47,0.67) -- (0.49,0.66) -- (0.51,0.65) -- (0.54,0.65) -- (0.57,0.65) -- (0.59,0.65) ;
\draw [stroke] (0.9,0.59) -- (0.9,0.59) -- (0.89,0.58) -- (0.88,0.58) -- (0.87,0.58) -- (0.86,0.58) -- (0.85,0.57) -- (0.84,0.57) -- (0.82,0.56) -- (0.81,0.54) -- (0.79,0.52) -- (0.78,0.49) -- (0.77,0.47) -- (0.77,0.44) -- (0.76,0.42) -- (0.76,0.4) -- (0.76,0.39) -- (0.76,0.38) -- (0.77,0.37) -- (0.77,0.37) -- (0.78,0.37) -- (0.8,0.37) -- (0.82,0.37) -- (0.84,0.38) -- (0.86,0.39) -- (0.88,0.4) -- (0.9,0.42) -- (0.92,0.44) -- (0.93,0.46) -- (0.94,0.48) -- (0.95,0.5) -- (0.96,0.52) -- (0.96,0.54) -- (0.96,0.55) -- (0.96,0.57) -- (0.94,0.59) -- (0.94,0.6) -- (0.93,0.61) -- (0.91,0.62) -- (0.9,0.62) -- (0.9,0.61) -- (0.89,0.6) -- (0.88,0.59) -- (0.87,0.58) -- (0.87,0.56) ;
\draw [stroke] (1.23,1.33) -- (1.23,1.33) -- (1.23,1.33) -- (1.23,1.33) -- (1.23,1.33) -- (1.24,1.33) -- (1.25,1.33) -- (1.26,1.33) -- (1.27,1.33) -- (1.29,1.34) -- (1.3,1.34) -- (1.32,1.34) -- (1.33,1.34) -- (1.35,1.34) -- (1.36,1.33) -- (1.37,1.33) -- (1.38,1.32) -- (1.38,1.31) -- (1.39,1.3) -- (1.39,1.28) -- (1.39,1.27) -- (1.38,1.24) -- (1.37,1.22) -- (1.36,1.19) -- (1.34,1.16) -- (1.32,1.14) -- (1.3,1.12) -- (1.28,1.09) -- (1.26,1.07) -- (1.24,1.05) -- (1.22,1.03) -- (1.21,1.02) -- (1.2,1.01) -- (1.19,1.0) -- (1.19,1.0) -- (1.19,1.0) -- (1.2,1.0) -- (1.2,1.0) -- (1.21,1.0) -- (1.22,1.0) -- (1.23,0.99) -- (1.25,0.99) -- (1.27,1.0) -- (1.3,1.0) -- (1.33,1.01) -- (1.36,1.02) -- (1.39,1.04) ;
\draw [stroke] (1.63,0.74) -- (1.62,0.74) -- (1.62,0.74) -- (1.62,0.74) -- (1.63,0.74) -- (1.63,0.74) -- (1.63,0.74) -- (1.64,0.74) -- (1.64,0.74) -- (1.66,0.74) -- (1.68,0.74) -- (1.7,0.74) -- (1.73,0.74) -- (1.76,0.74) -- (1.79,0.74) -- (1.82,0.74) -- (1.86,0.74) -- (1.89,0.74) -- (1.93,0.74) -- (1.96,0.73) -- (1.99,0.73) -- (2.02,0.73) -- (2.04,0.72) ;
\draw [stroke] (1.95,0.86) -- (1.94,0.86) -- (1.93,0.85) -- (1.93,0.85) -- (1.92,0.83) -- (1.92,0.82) -- (1.91,0.79) -- (1.91,0.77) -- (1.92,0.74) -- (1.92,0.7) -- (1.93,0.66) -- (1.94,0.62) -- (1.94,0.58) -- (1.95,0.54) -- (1.96,0.5) -- (1.97,0.47) -- (1.99,0.45) ;
\draw [stroke] (2.31,0.85) -- (2.31,0.85) -- (2.32,0.85) -- (2.32,0.85) -- (2.33,0.85) -- (2.35,0.86) -- (2.36,0.86) -- (2.38,0.86) -- (2.4,0.86) -- (2.41,0.86) -- (2.43,0.85) -- (2.44,0.84) -- (2.45,0.82) -- (2.47,0.8) -- (2.47,0.77) -- (2.47,0.74) -- (2.46,0.7) -- (2.45,0.65) -- (2.44,0.61) -- (2.42,0.57) -- (2.4,0.54) -- (2.38,0.5) -- (2.36,0.47) -- (2.34,0.45) -- (2.33,0.43) -- (2.32,0.42) -- (2.3,0.42) -- (2.3,0.43) -- (2.3,0.44) ;
\draw [stroke] (2.75,0.79) -- (2.76,0.8) -- (2.76,0.8) -- (2.76,0.8) -- (2.76,0.8) -- (2.76,0.8) -- (2.76,0.8) -- (2.75,0.8) -- (2.75,0.81) -- (2.75,0.81) -- (2.74,0.81) -- (2.72,0.82) -- (2.71,0.82) -- (2.69,0.82) -- (2.66,0.82) -- (2.64,0.81) -- (2.62,0.8) -- (2.59,0.78) -- (2.56,0.76) -- (2.54,0.73) -- (2.53,0.7) -- (2.52,0.67) -- (2.52,0.65) -- (2.53,0.62) -- (2.54,0.59) -- (2.55,0.56) -- (2.58,0.55) -- (2.61,0.53) -- (2.65,0.52) -- (2.69,0.51) -- (2.74,0.52) ;
\draw [stroke] (2.93,0.24) -- (2.93,0.24) -- (2.94,0.24) -- (2.94,0.24) -- (2.95,0.24) -- (2.96,0.25) -- (2.97,0.27) -- (3.0,0.3) -- (3.02,0.33) -- (3.05,0.37) -- (3.08,0.4) -- (3.1,0.43) -- (3.12,0.46) -- (3.13,0.47) -- (3.15,0.48) -- (3.16,0.49) -- (3.16,0.49) -- (3.17,0.48) -- (3.17,0.48) -- (3.17,0.47) -- (3.17,0.45) -- (3.17,0.43) -- (3.16,0.41) -- (3.16,0.38) -- (3.15,0.35) -- (3.15,0.32) -- (3.15,0.3) -- (3.14,0.28) -- (3.14,0.26) -- (3.15,0.25) -- (3.15,0.24) -- (3.15,0.23) -- (3.16,0.23) ;
\draw [stroke] (3.39,1.25) -- (3.4,1.26) -- (3.4,1.26) -- (3.41,1.27) -- (3.42,1.28) -- (3.43,1.29) -- (3.45,1.29) -- (3.47,1.3) -- (3.49,1.3) -- (3.52,1.31) -- (3.54,1.31) -- (3.57,1.32) -- (3.6,1.32) -- (3.62,1.33) -- (3.65,1.33) -- (3.67,1.33) -- (3.69,1.33) -- (3.7,1.33) -- (3.71,1.32) -- (3.71,1.31) -- (3.71,1.29) -- (3.69,1.27) -- (3.68,1.24) -- (3.65,1.2) -- (3.62,1.17) -- (3.59,1.13) -- (3.56,1.1) -- (3.53,1.07) -- (3.5,1.04) -- (3.48,1.03) -- (3.47,1.01) -- (3.46,1.0) -- (3.46,1.0) -- (3.46,1.0) -- (3.47,1.0) -- (3.48,1.0) -- (3.5,1.0) -- (3.52,1.0) -- (3.55,1.0) -- (3.59,1.0) -- (3.62,1.01) -- (3.66,1.02) -- (3.7,1.03) -- (3.73,1.04) -- (3.76,1.04) -- (3.8,1.05) -- (3.83,1.06) ;
\draw [stroke] (4.06,0.64) -- (4.06,0.65) -- (4.06,0.65) -- (4.06,0.65) -- (4.06,0.65) -- (4.06,0.65) -- (4.06,0.65) -- (4.07,0.65) -- (4.07,0.65) -- (4.09,0.65) -- (4.11,0.65) -- (4.14,0.65) -- (4.17,0.64) -- (4.21,0.64) -- (4.25,0.64) -- (4.3,0.64) -- (4.34,0.64) -- (4.38,0.65) -- (4.42,0.65) -- (4.46,0.66) -- (4.49,0.67) ;
\draw [stroke] (4.4,0.88) -- (4.39,0.88) -- (4.38,0.87) -- (4.38,0.86) -- (4.38,0.85) -- (4.38,0.82) -- (4.38,0.8) -- (4.38,0.76) -- (4.38,0.73) -- (4.38,0.69) -- (4.38,0.64) -- (4.38,0.6) -- (4.38,0.56) -- (4.38,0.53) -- (4.39,0.49) -- (4.39,0.46) -- (4.4,0.43) -- (4.4,0.4) -- (4.41,0.38) -- (4.42,0.37) ;
\draw [stroke] (4.96,0.85) -- (4.97,0.85) -- (4.98,0.85) -- (4.98,0.85) -- (4.99,0.84) -- (5.0,0.84) -- (5.0,0.84) -- (5.01,0.83) -- (5.02,0.82) -- (5.03,0.81) -- (5.03,0.8) -- (5.04,0.79) -- (5.04,0.77) -- (5.04,0.75) -- (5.04,0.73) -- (5.03,0.7) -- (5.02,0.67) -- (5.01,0.65) -- (4.99,0.62) -- (4.97,0.6) -- (4.95,0.58) -- (4.94,0.57) -- (4.92,0.55) -- (4.9,0.54) -- (4.89,0.53) -- (4.88,0.52) -- (4.87,0.53) ;
\draw [stroke] (5.3,0.84) -- (5.3,0.84) -- (5.3,0.84) -- (5.3,0.85) -- (5.29,0.85) -- (5.29,0.85) -- (5.29,0.85) -- (5.28,0.86) -- (5.27,0.86) -- (5.26,0.86) -- (5.25,0.86) -- (5.23,0.86) -- (5.21,0.85) -- (5.19,0.83) -- (5.17,0.81) -- (5.16,0.78) -- (5.15,0.76) -- (5.13,0.73) -- (5.13,0.71) -- (5.13,0.68) -- (5.13,0.66) -- (5.13,0.64) -- (5.14,0.62) -- (5.15,0.61) -- (5.17,0.59) -- (5.18,0.58) -- (5.21,0.58) -- (5.23,0.58) -- (5.25,0.58) -- (5.27,0.59) ;
\draw [stroke] (5.36,0.33) -- (5.37,0.34) -- (5.37,0.34) -- (5.38,0.35) -- (5.39,0.35) -- (5.4,0.35) -- (5.41,0.35) -- (5.42,0.35) -- (5.43,0.36) -- (5.44,0.36) -- (5.46,0.36) -- (5.47,0.36) -- (5.49,0.36) -- (5.5,0.36) -- (5.51,0.36) -- (5.52,0.36) -- (5.53,0.36) -- (5.53,0.35) -- (5.53,0.35) -- (5.53,0.35) -- (5.53,0.34) -- (5.53,0.33) -- (5.52,0.31) -- (5.52,0.29) -- (5.5,0.27) -- (5.49,0.25) -- (5.48,0.24) -- (5.46,0.22) -- (5.45,0.2) -- (5.44,0.19) -- (5.42,0.18) -- (5.41,0.17) -- (5.39,0.17) -- (5.38,0.16) -- (5.37,0.16) -- (5.37,0.16) -- (5.36,0.16) -- (5.36,0.16) -- (5.36,0.16) -- (5.37,0.16) -- (5.37,0.16) -- (5.38,0.15) -- (5.39,0.15) -- (5.4,0.15) -- (5.41,0.15) -- (5.43,0.15) -- (5.46,0.15) -- (5.48,0.16) -- (5.51,0.16) -- (5.55,0.18) -- (5.58,0.2) ;
\draw [stroke] (5.93,1.47) -- (5.94,1.47) -- (5.94,1.47) -- (5.95,1.48) -- (5.97,1.48) -- (5.99,1.48) -- (6.01,1.48) -- (6.03,1.48) -- (6.05,1.47) -- (6.06,1.47) -- (6.08,1.46) -- (6.1,1.46) -- (6.11,1.44) -- (6.12,1.43) -- (6.12,1.41) -- (6.13,1.39) -- (6.12,1.37) -- (6.11,1.34) -- (6.1,1.31) -- (6.08,1.28) -- (6.06,1.26) -- (6.04,1.23) -- (6.03,1.22) -- (6.01,1.2) -- (6.0,1.19) -- (5.99,1.18) -- (5.98,1.17) -- (5.98,1.17) -- (5.98,1.17) -- (5.99,1.17) -- (5.99,1.16) -- (6.0,1.16) -- (6.01,1.16) -- (6.03,1.16) -- (6.05,1.17) -- (6.07,1.17) -- (6.1,1.17) -- (6.13,1.18) -- (6.16,1.18) -- (6.2,1.19) -- (6.23,1.19) -- (6.27,1.2) ;
\draw [stroke] (6.32,0.67) -- (6.32,0.67) -- (6.32,0.67) -- (6.32,0.67) -- (6.33,0.67) -- (6.34,0.66) -- (6.35,0.66) -- (6.38,0.66) -- (6.41,0.66) -- (6.45,0.66) -- (6.49,0.67) -- (6.54,0.67) -- (6.59,0.68) -- (6.64,0.7) -- (6.68,0.71) -- (6.71,0.73) ;
\draw [stroke] (6.61,0.83) -- (6.6,0.82) -- (6.59,0.81) -- (6.59,0.8) -- (6.59,0.78) -- (6.59,0.76) -- (6.59,0.73) -- (6.59,0.69) -- (6.6,0.66) -- (6.61,0.63) -- (6.62,0.59) -- (6.63,0.55) -- (6.64,0.52) -- (6.65,0.48) -- (6.66,0.46) ;
\draw [stroke] (7.19,0.86) -- (7.19,0.86) -- (7.19,0.86) -- (7.2,0.86) -- (7.2,0.86) -- (7.21,0.86) -- (7.22,0.86) -- (7.23,0.86) -- (7.25,0.86) -- (7.26,0.86) -- (7.28,0.86) -- (7.29,0.85) -- (7.29,0.85) -- (7.3,0.84) -- (7.31,0.83) -- (7.32,0.81) -- (7.32,0.79) -- (7.32,0.76) -- (7.32,0.74) -- (7.31,0.71) -- (7.29,0.68) -- (7.28,0.65) -- (7.26,0.62) -- (7.24,0.6) -- (7.22,0.58) -- (7.2,0.57) -- (7.19,0.56) -- (7.17,0.56) -- (7.17,0.56) ;
\draw [stroke] (7.55,0.89) -- (7.55,0.89) -- (7.54,0.89) -- (7.53,0.88) -- (7.52,0.88) -- (7.51,0.88) -- (7.5,0.88) -- (7.49,0.87) -- (7.48,0.87) -- (7.47,0.86) -- (7.45,0.85) -- (7.44,0.84) -- (7.43,0.82) -- (7.42,0.8) -- (7.41,0.78) -- (7.41,0.76) -- (7.41,0.74) -- (7.42,0.72) -- (7.43,0.7) -- (7.44,0.69) -- (7.46,0.67) -- (7.48,0.65) -- (7.5,0.64) -- (7.52,0.63) -- (7.54,0.63) ;
\draw [stroke] (7.7,0.49) -- (7.71,0.49) -- (7.71,0.49) -- (7.72,0.49) -- (7.73,0.49) -- (7.74,0.49) -- (7.75,0.49) -- (7.77,0.49) -- (7.79,0.49) -- (7.8,0.49) -- (7.82,0.49) -- (7.83,0.48) -- (7.84,0.48) -- (7.85,0.47) -- (7.85,0.47) -- (7.86,0.46) -- (7.86,0.44) -- (7.85,0.43) -- (7.85,0.42) -- (7.84,0.4) -- (7.83,0.38) -- (7.81,0.36) -- (7.8,0.34) -- (7.78,0.33) -- (7.76,0.31) -- (7.75,0.29) -- (7.74,0.28) -- (7.73,0.26) -- (7.72,0.25) -- (7.72,0.25) -- (7.72,0.25) -- (7.72,0.25) -- (7.72,0.25) -- (7.72,0.26) -- (7.73,0.26) -- (7.74,0.27) -- (7.76,0.29) -- (7.77,0.3) -- (7.79,0.32) -- (7.81,0.35) -- (7.83,0.37) -- (7.84,0.39) -- (7.86,0.41) -- (7.87,0.43) -- (7.88,0.44) -- (7.89,0.46) -- (7.89,0.47) -- (7.89,0.48) -- (7.89,0.49) -- (7.89,0.5) -- (7.88,0.51) -- (7.87,0.52) -- (7.86,0.52) -- (7.86,0.53) -- (7.85,0.54) -- (7.84,0.54) -- (7.83,0.54) -- (7.82,0.54) -- (7.81,0.54) -- (7.8,0.54) -- (7.79,0.54) -- (7.79,0.53) -- (7.79,0.53) -- (7.79,0.53) -- (7.79,0.53) -- (7.79,0.53) -- (7.8,0.53) -- (7.8,0.53) -- (7.81,0.52) -- (7.82,0.52) -- (7.83,0.52) -- (7.85,0.52) -- (7.87,0.52) -- (7.88,0.52) -- (7.89,0.51) -- (7.9,0.51) -- (7.91,0.51) -- (7.92,0.51) -- (7.93,0.5) -- (7.94,0.5) -- (7.94,0.5) -- (7.94,0.5) -- (7.94,0.5) -- (7.94,0.49) -- (7.93,0.49) -- (7.93,0.49) -- (7.92,0.48) -- (7.91,0.47) -- (7.9,0.46) -- (7.9,0.45) -- (7.89,0.44) -- (7.88,0.43) -- (7.87,0.42) -- (7.87,0.41) -- (7.86,0.4) -- (7.86,0.39) -- (7.86,0.39) -- (7.86,0.39) -- (7.86,0.39) -- (7.87,0.38) -- (7.87,0.38) -- (7.87,0.38) -- (7.88,0.37) -- (7.89,0.37) -- (7.89,0.36) -- (7.89,0.36) -- (7.9,0.36) -- (7.9,0.35) -- (7.9,0.35) -- (7.9,0.34) -- (7.91,0.33) -- (7.91,0.32) -- (7.91,0.31) -- (7.91,0.3) -- (7.91,0.29) -- (7.91,0.28) -- (7.91,0.27) -- (7.9,0.26) -- (7.9,0.25) -- (7.9,0.24) -- (7.89,0.24) -- (7.89,0.23) -- (7.88,0.22) -- (7.88,0.21) -- (7.87,0.21) -- (7.87,0.21) -- (7.86,0.2) -- (7.86,0.2) -- (7.86,0.2) -- (7.86,0.2) -- (7.86,0.2) -- (7.86,0.2) -- (7.86,0.2) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.22) -- (7.86,0.21) -- (7.86,0.21) -- (7.86,0.21) -- (7.87,0.21) -- (7.87,0.21) -- (7.87,0.21) -- (7.87,0.21) -- (7.87,0.21) -- (7.87,0.21) -- (7.87,0.22) ;
\draw [stroke] (7.78,0.49) -- (7.79,0.49) -- (7.79,0.49) -- (7.79,0.49) -- (7.79,0.49) -- (7.8,0.49) -- (7.8,0.49) -- (7.8,0.49) -- (7.81,0.49) -- (7.81,0.49) -- (7.82,0.49) -- (7.83,0.49) -- (7.84,0.49) -- (7.85,0.49) -- (7.86,0.49) -- (7.87,0.48) -- (7.88,0.48) -- (7.89,0.48) -- (7.9,0.47) -- (7.9,0.47) -- (7.91,0.46) -- (7.91,0.46) -- (7.91,0.45) -- (7.91,0.44) -- (7.91,0.43) -- (7.91,0.42) -- (7.9,0.4) -- (7.9,0.39) -- (7.89,0.37) -- (7.88,0.35) -- (7.87,0.34) -- (7.87,0.33) -- (7.86,0.33) -- (7.85,0.32) -- (7.84,0.32) -- (7.84,0.31) -- (7.83,0.31) -- (7.83,0.31) -- (7.83,0.31) -- (7.82,0.31) -- (7.82,0.31) -- (7.82,0.31) -- (7.82,0.31) -- (7.82,0.31) -- (7.82,0.31) -- (7.82,0.31) -- (7.82,0.31) -- (7.83,0.31) -- (7.83,0.31) -- (7.83,0.31) -- (7.84,0.31) -- (7.85,0.31) -- (7.85,0.31) -- (7.85,0.31) -- (7.86,0.31) -- (7.86,0.31) -- (7.86,0.31) -- (7.87,0.31) -- (7.87,0.31) -- (7.87,0.31) -- (7.87,0.3) -- (7.88,0.29) -- (7.89,0.28) -- (7.89,0.26) -- (7.9,0.24) -- (7.9,0.22) -- (7.9,0.21) -- (7.9,0.2) -- (7.9,0.19) -- (7.9,0.17) -- (7.89,0.16) -- (7.88,0.13) -- (7.87,0.11) -- (7.86,0.09) -- (7.85,0.07) -- (7.84,0.06) -- (7.82,0.04) -- (7.8,0.02) -- (7.78,0.01) -- (7.76,0.0) -- (7.74,0.0) -- (7.73,0.01) ;
\draw [stroke] (8.17,1.38) -- (8.17,1.38) -- (8.18,1.39) -- (8.19,1.39) -- (8.2,1.39) -- (8.21,1.4) -- (8.23,1.4) -- (8.24,1.41) -- (8.26,1.41) -- (8.28,1.41) -- (8.3,1.41) -- (8.32,1.41) -- (8.33,1.4) -- (8.34,1.39) -- (8.35,1.38) -- (8.35,1.37) -- (8.35,1.36) -- (8.35,1.34) -- (8.34,1.31) -- (8.32,1.28) -- (8.31,1.25) -- (8.28,1.22) -- (8.25,1.19) -- (8.23,1.17) -- (8.2,1.15) -- (8.18,1.13) -- (8.17,1.11) -- (8.15,1.1) -- (8.15,1.09) -- (8.14,1.08) -- (8.14,1.08) -- (8.14,1.07) -- (8.15,1.07) -- (8.15,1.07) -- (8.16,1.07) -- (8.18,1.06) -- (8.2,1.06) -- (8.23,1.05) -- (8.27,1.05) -- (8.31,1.04) -- (8.35,1.04) -- (8.4,1.05) ;
\draw [stroke] (8.78,0.72) -- (8.77,0.73) -- (8.77,0.73) -- (8.78,0.73) -- (8.78,0.72) -- (8.78,0.72) -- (8.79,0.72) -- (8.8,0.71) -- (8.82,0.71) -- (8.85,0.71) -- (8.88,0.7) -- (8.92,0.7) -- (8.95,0.7) -- (9.0,0.7) -- (9.04,0.71) -- (9.09,0.71) ;
\draw [stroke] (8.82,0.45) -- (8.82,0.45) -- (8.82,0.45) -- (8.82,0.45) -- (8.83,0.45) -- (8.84,0.44) -- (8.86,0.44) -- (8.88,0.44) -- (8.92,0.44) -- (8.96,0.44) -- (9.0,0.45) -- (9.05,0.45) -- (9.09,0.46) -- (9.14,0.47) -- (9.18,0.48) ;
\draw [stroke] (9.68,0.73) -- (9.68,0.73) -- (9.69,0.74) -- (9.69,0.74) -- (9.69,0.74) -- (9.71,0.75) -- (9.73,0.77) -- (9.76,0.8) -- (9.8,0.83) -- (9.83,0.87) -- (9.87,0.91) -- (9.9,0.94) -- (9.93,0.97) -- (9.95,0.99) -- (9.97,1.01) -- (9.98,1.02) -- (9.99,1.03) -- (10.0,1.03) -- (10.0,1.02) -- (10.0,1.0) -- (10.0,0.97) -- (9.99,0.94) -- (9.99,0.89) -- (9.98,0.85) -- (9.97,0.8) -- (9.96,0.75) -- (9.96,0.69) -- (9.95,0.63) -- (9.95,0.58) -- (9.94,0.53) -- (9.94,0.48) -- (9.94,0.44) -- (9.95,0.41) -- (9.95,0.38) ;

		   \end{tikzpicture}

==> 2920.tex <==

	\tikzset{stroke/.style={black, line width=0.1mm}}

	\begin{tikzpicture}
\draw [stroke] (0.48,1.65) -- (0.48,1.66) -- (0.47,1.67) -- (0.47,1.69) -- (0.47,1.7) -- (0.47,1.71) -- (0.46,1.72) -- (0.46,1.74) -- (0.45,1.75) -- (0.44,1.77) -- (0.43,1.78) -- (0.42,1.79) -- (0.4,1.81) -- (0.39,1.81) -- (0.37,1.82) -- (0.34,1.82) -- (0.32,1.82) -- (0.3,1.81) -- (0.27,1.8) -- (0.24,1.78) -- (0.21,1.75) -- (0.17,1.72) -- (0.14,1.68) -- (0.11,1.64) -- (0.08,1.6) -- (0.05,1.55) -- (0.03,1.5) -- (0.02,1.45) -- (0.0,1.4) -- (0.0,1.35) -- (0.0,1.3) -- (0.0,1.26) -- (0.01,1.22) -- (0.02,1.17) -- (0.04,1.13) -- (0.05,1.09) -- (0.08,1.05) -- (0.1,1.02) -- (0.13,0.99) -- (0.17,0.97) -- (0.21,0.95) -- (0.25,0.94) -- (0.31,0.93) -- (0.36,0.93) ;
\draw [stroke] (0.79,1.2) -- (0.79,1.2) -- (0.79,1.2) -- (0.79,1.19) -- (0.79,1.18) -- (0.79,1.16) -- (0.78,1.15) -- (0.78,1.13) -- (0.78,1.11) -- (0.77,1.08) -- (0.77,1.06) -- (0.77,1.03) -- (0.77,1.0) -- (0.77,0.97) -- (0.77,0.95) -- (0.77,0.92) -- (0.76,0.89) -- (0.76,0.87) -- (0.76,0.84) -- (0.76,0.82) -- (0.75,0.79) -- (0.75,0.76) -- (0.74,0.74) -- (0.74,0.72) -- (0.73,0.71) -- (0.73,0.69) -- (0.72,0.69) -- (0.72,0.68) -- (0.72,0.68) -- (0.72,0.68) -- (0.72,0.68) -- (0.72,0.68) -- (0.73,0.69) -- (0.73,0.69) -- (0.73,0.7) -- (0.73,0.71) -- (0.74,0.73) -- (0.75,0.75) -- (0.75,0.77) -- (0.76,0.78) -- (0.76,0.79) -- (0.77,0.8) -- (0.77,0.81) -- (0.77,0.82) -- (0.77,0.83) -- (0.78,0.84) -- (0.79,0.85) -- (0.79,0.87) -- (0.8,0.88) -- (0.81,0.9) -- (0.82,0.91) -- (0.83,0.93) -- (0.84,0.95) -- (0.85,0.97) -- (0.86,0.98) -- (0.87,1.0) -- (0.87,1.01) ;
\draw [stroke] (0.85,0.95) -- (0.86,0.96) -- (0.87,0.97) -- (0.88,0.98) -- (0.9,0.99) -- (0.91,1.0) -- (0.93,1.01) -- (0.94,1.02) -- (0.95,1.03) -- (0.96,1.04) -- (0.97,1.05) -- (0.98,1.05) -- (0.98,1.05) -- (0.99,1.05) -- (0.99,1.05) -- (0.99,1.05) -- (0.99,1.05) -- (0.99,1.04) -- (0.99,1.04) -- (1.0,1.03) -- (1.01,1.01) -- (1.02,1.0) -- (1.02,0.99) -- (1.02,0.97) -- (1.03,0.96) -- (1.03,0.94) -- (1.03,0.93) -- (1.03,0.92) -- (1.02,0.9) -- (1.01,0.89) -- (1.01,0.87) -- (1.0,0.86) -- (0.99,0.85) -- (0.98,0.85) -- (0.97,0.84) -- (0.97,0.84) -- (0.96,0.84) -- (0.96,0.84) -- (0.95,0.84) -- (0.94,0.85) -- (0.93,0.85) -- (0.92,0.85) -- (0.91,0.86) -- (0.9,0.86) -- (0.89,0.86) -- (0.89,0.86) -- (0.88,0.86) -- (0.88,0.86) -- (0.88,0.86) -- (0.87,0.86) -- (0.87,0.86) -- (0.87,0.86) -- (0.87,0.86) -- (0.88,0.86) -- (0.88,0.86) -- (0.88,0.86) -- (0.88,0.86) -- (0.88,0.86) -- (0.88,0.86) -- (0.89,0.86) -- (0.89,0.86) -- (0.89,0.86) -- (0.89,0.86) -- (0.89,0.86) -- (0.89,0.86) -- (0.89,0.86) -- (0.89,0.86) -- (0.9,0.86) -- (0.9,0.86) -- (0.9,0.85) -- (0.9,0.85) -- (0.91,0.85) -- (0.92,0.84) -- (0.92,0.83) -- (0.93,0.83) -- (0.93,0.82) -- (0.94,0.81) -- (0.95,0.8) -- (0.96,0.79) -- (0.97,0.78) -- (0.98,0.77) -- (0.99,0.76) -- (1.0,0.75) -- (1.02,0.74) -- (1.03,0.73) -- (1.04,0.72) -- (1.06,0.71) -- (1.07,0.69) -- (1.08,0.67) -- (1.09,0.66) -- (1.1,0.65) -- (1.11,0.64) -- (1.11,0.63) -- (1.12,0.62) -- (1.12,0.62) ;
\draw [stroke] (1.89,1.15) -- (1.9,1.15) -- (1.9,1.15) -- (1.9,1.15) -- (1.9,1.15) -- (1.9,1.15) -- (1.9,1.15) -- (1.91,1.15) -- (1.91,1.15) -- (1.91,1.15) -- (1.91,1.15) -- (1.91,1.15) -- (1.91,1.15) -- (1.92,1.14) -- (1.92,1.14) -- (1.93,1.14) -- (1.94,1.15) -- (1.96,1.15) -- (1.99,1.15) -- (2.04,1.15) -- (2.09,1.15) -- (2.16,1.16) -- (2.22,1.17) -- (2.28,1.18) -- (2.33,1.19) -- (2.37,1.19) -- (2.41,1.2) -- (2.43,1.2) -- (2.46,1.19) -- (2.47,1.19) -- (2.48,1.17) -- (2.47,1.16) ;
\draw [stroke] (1.95,0.84) -- (1.96,0.84) -- (1.96,0.84) -- (1.96,0.83) -- (1.97,0.83) -- (1.98,0.83) -- (1.99,0.83) -- (2.02,0.83) -- (2.05,0.83) -- (2.09,0.83) -- (2.14,0.84) -- (2.19,0.85) -- (2.24,0.86) -- (2.29,0.86) -- (2.33,0.87) -- (2.36,0.88) ;
\draw [stroke] (3.27,1.59) -- (3.27,1.59) -- (3.26,1.59) -- (3.26,1.58) -- (3.26,1.57) -- (3.27,1.56) -- (3.27,1.54) -- (3.27,1.52) -- (3.27,1.5) -- (3.27,1.48) -- (3.27,1.45) -- (3.27,1.43) -- (3.27,1.4) -- (3.27,1.37) -- (3.27,1.34) -- (3.27,1.31) -- (3.27,1.28) -- (3.26,1.25) -- (3.26,1.23) -- (3.25,1.2) -- (3.25,1.18) -- (3.24,1.16) -- (3.23,1.14) ;
\draw [stroke] (2.74,0.86) -- (2.74,0.86) -- (2.75,0.86) -- (2.75,0.86) -- (2.75,0.86) -- (2.76,0.86) -- (2.76,0.87) -- (2.78,0.87) -- (2.8,0.88) -- (2.82,0.88) -- (2.86,0.89) -- (2.9,0.89) -- (2.95,0.9) -- (3.0,0.9) -- (3.07,0.91) -- (3.15,0.92) -- (3.23,0.93) -- (3.3,0.94) -- (3.38,0.95) -- (3.45,0.95) -- (3.51,0.96) ;
\draw [stroke] (3.08,0.67) -- (3.08,0.67) -- (3.08,0.67) -- (3.08,0.67) -- (3.09,0.67) -- (3.1,0.68) -- (3.11,0.68) -- (3.13,0.69) -- (3.15,0.69) -- (3.17,0.69) -- (3.2,0.69) -- (3.23,0.69) -- (3.26,0.69) -- (3.28,0.69) -- (3.3,0.69) -- (3.31,0.69) -- (3.32,0.68) -- (3.32,0.67) -- (3.32,0.67) -- (3.33,0.65) -- (3.33,0.64) -- (3.33,0.62) -- (3.33,0.61) -- (3.32,0.59) -- (3.32,0.56) -- (3.31,0.54) -- (3.3,0.51) -- (3.28,0.48) -- (3.26,0.44) -- (3.23,0.4) -- (3.2,0.37) -- (3.16,0.33) -- (3.12,0.3) -- (3.09,0.26) -- (3.06,0.23) -- (3.04,0.21) -- (3.02,0.19) -- (3.01,0.16) -- (3.0,0.14) -- (2.99,0.12) -- (2.99,0.1) -- (2.98,0.08) -- (2.99,0.07) -- (2.99,0.06) -- (3.0,0.05) -- (3.02,0.04) -- (3.03,0.03) -- (3.05,0.03) -- (3.09,0.02) -- (3.13,0.01) -- (3.19,0.0) -- (3.24,0.0) -- (3.3,0.0) -- (3.35,0.0) -- (3.41,0.01) -- (3.47,0.02) ;
\draw [stroke] (4.58,1.03) -- (4.59,1.02) -- (4.59,1.02) -- (4.58,1.02) -- (4.58,1.02) -- (4.58,1.02) -- (4.59,1.02) -- (4.59,1.02) -- (4.59,1.02) -- (4.59,1.02) -- (4.6,1.02) -- (4.6,1.02) -- (4.6,1.02) -- (4.6,1.02) -- (4.6,1.02) -- (4.6,1.02) -- (4.61,1.02) -- (4.61,1.02) -- (4.61,1.02) -- (4.62,1.02) -- (4.62,1.02) -- (4.63,1.02) -- (4.65,1.03) -- (4.67,1.03) -- (4.7,1.03) -- (4.73,1.03) -- (4.77,1.04) -- (4.79,1.04) -- (4.82,1.04) -- (4.84,1.04) -- (4.87,1.05) -- (4.89,1.05) -- (4.91,1.05) -- (4.94,1.05) -- (4.97,1.05) -- (4.99,1.05) -- (5.01,1.05) -- (5.01,1.05) -- (5.01,1.05) -- (5.01,1.05) -- (5.01,1.05) -- (5.01,1.05) -- (5.01,1.05) -- (5.01,1.05) -- (5.01,1.05) -- (5.01,1.05) -- (5.01,1.05) -- (5.01,1.05) -- (5.0,1.05) -- (5.0,1.05) -- (5.0,1.05) -- (5.0,1.05) -- (5.0,1.06) -- (5.0,1.06) -- (5.0,1.06) -- (4.99,1.06) -- (4.99,1.06) -- (4.98,1.07) -- (4.96,1.07) ;
\draw [stroke] (5.34,1.18) -- (5.34,1.18) -- (5.34,1.18) -- (5.35,1.18) -- (5.35,1.18) -- (5.35,1.18) -- (5.36,1.18) -- (5.37,1.18) -- (5.4,1.2) -- (5.42,1.21) -- (5.46,1.23) -- (5.5,1.25) -- (5.53,1.27) -- (5.57,1.3) -- (5.6,1.32) -- (5.63,1.35) -- (5.65,1.38) -- (5.67,1.4) -- (5.69,1.43) -- (5.7,1.45) -- (5.71,1.47) -- (5.72,1.49) -- (5.72,1.51) -- (5.72,1.53) -- (5.73,1.53) -- (5.73,1.54) -- (5.72,1.54) -- (5.72,1.54) -- (5.72,1.54) -- (5.72,1.53) -- (5.71,1.52) -- (5.71,1.51) -- (5.7,1.48) -- (5.69,1.45) -- (5.68,1.42) -- (5.67,1.38) -- (5.66,1.34) -- (5.65,1.3) -- (5.65,1.27) -- (5.65,1.23) -- (5.65,1.19) -- (5.65,1.16) -- (5.65,1.12) -- (5.65,1.09) -- (5.65,1.06) -- (5.65,1.03) -- (5.65,1.01) -- (5.65,0.99) -- (5.65,0.97) -- (5.65,0.95) -- (5.65,0.95) -- (5.65,0.95) -- (5.65,0.95) ;
\draw [stroke] (4.38,1.47) -- (4.38,1.45) -- (4.37,1.43) -- (4.36,1.41) -- (4.35,1.38) -- (4.34,1.34) -- (4.33,1.29) -- (4.33,1.24) -- (4.32,1.19) -- (4.32,1.14) -- (4.32,1.08) -- (4.31,1.02) -- (4.31,0.95) -- (4.31,0.89) -- (4.32,0.82) -- (4.33,0.76) -- (4.34,0.7) -- (4.36,0.64) -- (4.39,0.58) ;
\draw [stroke] (6.05,1.76) -- (6.07,1.75) -- (6.09,1.74) -- (6.1,1.72) -- (6.12,1.69) -- (6.13,1.66) -- (6.15,1.62) -- (6.16,1.57) -- (6.17,1.51) -- (6.19,1.45) -- (6.2,1.38) -- (6.2,1.31) -- (6.2,1.24) -- (6.2,1.17) -- (6.2,1.1) -- (6.19,1.02) -- (6.17,0.95) -- (6.15,0.88) -- (6.12,0.82) -- (6.09,0.75) -- (6.06,0.69) -- (6.01,0.62) ;
\draw [stroke] (6.8,2.02) -- (6.8,2.01) -- (6.8,2.0) -- (6.8,1.99) -- (6.8,1.97) -- (6.8,1.94) -- (6.8,1.92) -- (6.81,1.89) -- (6.81,1.85) -- (6.81,1.82) -- (6.81,1.79) -- (6.81,1.76) -- (6.81,1.73) -- (6.81,1.7) -- (6.81,1.68) -- (6.81,1.66) -- (6.8,1.65) -- (6.8,1.64) -- (6.8,1.63) -- (6.8,1.62) -- (6.81,1.61) -- (6.81,1.61) -- (6.81,1.61) -- (6.81,1.61) -- (6.81,1.61) -- (6.81,1.61) -- (6.8,1.61) -- (6.8,1.62) -- (6.81,1.62) -- (6.81,1.62) -- (6.81,1.62) -- (6.81,1.62) -- (6.81,1.62) -- (6.81,1.63) -- (6.81,1.63) -- (6.82,1.63) -- (6.82,1.64) -- (6.82,1.65) -- (6.82,1.66) -- (6.82,1.67) -- (6.83,1.69) -- (6.84,1.71) -- (6.84,1.73) -- (6.85,1.75) -- (6.87,1.78) -- (6.88,1.8) -- (6.9,1.82) -- (6.91,1.84) -- (6.93,1.85) -- (6.94,1.86) -- (6.95,1.87) -- (6.95,1.87) -- (6.96,1.88) -- (6.96,1.88) -- (6.96,1.88) -- (6.96,1.88) -- (6.96,1.87) -- (6.96,1.87) -- (6.97,1.87) -- (6.98,1.87) -- (6.99,1.87) -- (6.99,1.86) -- (7.0,1.86) -- (7.01,1.85) -- (7.01,1.84) -- (7.02,1.83) -- (7.02,1.82) -- (7.02,1.81) -- (7.02,1.8) -- (7.02,1.79) -- (7.02,1.78) -- (7.02,1.77) -- (7.01,1.77) -- (7.01,1.76) -- (7.0,1.75) -- (6.99,1.74) -- (6.99,1.73) -- (6.98,1.73) -- (6.98,1.72) -- (6.97,1.72) -- (6.97,1.72) -- (6.96,1.72) -- (6.96,1.71) -- (6.96,1.71) -- (6.96,1.71) -- (6.96,1.71) -- (6.96,1.71) -- (6.96,1.71) -- (6.96,1.71) -- (6.96,1.71) -- (6.96,1.71) -- (6.96,1.71) -- (6.97,1.71) -- (6.97,1.71) -- (6.97,1.71) -- (6.97,1.71) -- (6.97,1.71) -- (6.97,1.71) -- (6.98,1.7) -- (6.98,1.7) -- (6.98,1.7) -- (6.99,1.7) -- (6.99,1.69) -- (7.0,1.69) -- (7.01,1.69) -- (7.01,1.68) -- (7.03,1.68) -- (7.04,1.67) -- (7.05,1.66) -- (7.06,1.66) -- (7.07,1.65) -- (7.08,1.64) -- (7.09,1.63) -- (7.1,1.62) -- (7.11,1.61) -- (7.11,1.61) -- (7.12,1.6) -- (7.13,1.59) -- (7.13,1.59) -- (7.14,1.58) -- (7.14,1.58) -- (7.14,1.58) -- (7.14,1.58) -- (7.14,1.58) -- (7.14,1.58) -- (7.14,1.58) -- (7.14,1.58) -- (7.14,1.58) -- (7.14,1.58) -- (7.14,1.58) -- (7.14,1.58) -- (7.14,1.58) -- (7.13,1.58) -- (7.13,1.58) -- (7.13,1.58) -- (7.13,1.59) -- (7.13,1.59) -- (7.13,1.59) -- (7.13,1.59) -- (7.12,1.59) -- (7.11,1.6) -- (7.11,1.61) ;
\draw [stroke] (7.46,1.8) -- (7.46,1.79) -- (7.46,1.79) -- (7.46,1.79) -- (7.45,1.79) -- (7.45,1.79) -- (7.46,1.8) -- (7.46,1.8) -- (7.46,1.79) -- (7.46,1.79) -- (7.46,1.79) -- (7.47,1.79) -- (7.47,1.79) -- (7.47,1.79) -- (7.47,1.79) -- (7.48,1.79) -- (7.49,1.79) -- (7.5,1.79) -- (7.51,1.78) -- (7.53,1.78) -- (7.55,1.78) -- (7.57,1.78) -- (7.59,1.78) -- (7.61,1.79) -- (7.63,1.79) -- (7.65,1.8) -- (7.67,1.81) -- (7.69,1.81) -- (7.71,1.82) ;
\draw [stroke] (7.63,1.93) -- (7.63,1.93) -- (7.63,1.92) -- (7.63,1.91) -- (7.63,1.9) -- (7.62,1.89) -- (7.63,1.87) -- (7.63,1.85) -- (7.63,1.83) -- (7.63,1.81) -- (7.63,1.79) -- (7.63,1.77) -- (7.63,1.75) -- (7.63,1.74) -- (7.63,1.72) -- (7.62,1.71) -- (7.62,1.7) -- (7.62,1.69) -- (7.62,1.68) -- (7.62,1.67) -- (7.62,1.67) -- (7.62,1.66) -- (7.62,1.66) -- (7.61,1.65) ;
\draw [stroke] (8.1,1.99) -- (8.1,1.99) -- (8.1,1.99) -- (8.1,1.99) -- (8.1,1.99) -- (8.1,1.99) -- (8.1,1.99) -- (8.1,1.99) -- (8.09,1.99) -- (8.09,1.99) -- (8.09,1.99) -- (8.09,1.99) -- (8.09,1.99) -- (8.09,1.99) -- (8.09,1.99) -- (8.09,1.99) -- (8.09,1.98) -- (8.09,1.99) -- (8.09,1.99) -- (8.1,1.99) -- (8.09,1.99) -- (8.1,1.98) -- (8.1,1.98) -- (8.09,1.98) -- (8.09,1.98) -- (8.09,1.98) -- (8.09,1.98) -- (8.09,1.97) -- (8.09,1.97) -- (8.09,1.97) -- (8.09,1.95) -- (8.09,1.94) -- (8.09,1.93) -- (8.09,1.92) -- (8.09,1.91) -- (8.08,1.89) -- (8.09,1.88) -- (8.08,1.86) -- (8.09,1.84) -- (8.09,1.82) -- (8.08,1.81) -- (8.08,1.79) -- (8.08,1.78) -- (8.08,1.76) -- (8.08,1.75) -- (8.08,1.74) -- (8.08,1.74) -- (8.08,1.73) -- (8.08,1.73) -- (8.08,1.72) -- (8.08,1.72) -- (8.08,1.72) -- (8.08,1.72) -- (8.08,1.72) -- (8.08,1.73) -- (8.08,1.73) -- (8.08,1.73) -- (8.08,1.73) -- (8.08,1.74) -- (8.08,1.74) -- (8.08,1.74) -- (8.07,1.74) -- (8.07,1.75) -- (8.07,1.76) -- (8.06,1.76) -- (8.05,1.77) ;
\draw [stroke] (8.88,1.49) -- (8.88,1.48) -- (8.88,1.46) -- (8.88,1.45) -- (8.88,1.43) -- (8.88,1.41) -- (8.88,1.38) -- (8.88,1.35) -- (8.88,1.32) -- (8.88,1.28) -- (8.88,1.24) -- (8.88,1.21) -- (8.88,1.17) -- (8.88,1.13) -- (8.88,1.1) -- (8.88,1.07) -- (8.88,1.05) -- (8.88,1.03) -- (8.89,1.01) -- (8.89,1.0) -- (8.89,0.99) -- (8.9,0.98) -- (8.9,0.98) -- (8.9,0.97) -- (8.9,0.97) -- (8.9,0.97) -- (8.9,0.97) -- (8.89,0.97) -- (8.89,0.97) -- (8.89,0.97) -- (8.89,0.97) -- (8.89,0.97) -- (8.89,0.97) -- (8.89,0.98) -- (8.89,0.98) -- (8.89,0.98) -- (8.89,0.99) -- (8.89,1.0) -- (8.89,1.01) -- (8.89,1.02) -- (8.89,1.04) -- (8.89,1.06) -- (8.89,1.08) -- (8.89,1.1) -- (8.89,1.13) -- (8.9,1.15) -- (8.9,1.16) -- (8.9,1.18) -- (8.91,1.19) -- (8.92,1.21) -- (8.93,1.22) -- (8.95,1.23) -- (8.96,1.24) -- (8.98,1.25) -- (8.99,1.26) -- (9.0,1.26) -- (9.01,1.27) -- (9.01,1.27) -- (9.02,1.27) -- (9.03,1.26) -- (9.05,1.26) -- (9.06,1.26) -- (9.08,1.25) -- (9.1,1.24) -- (9.11,1.23) -- (9.13,1.22) -- (9.14,1.2) -- (9.15,1.19) -- (9.16,1.18) -- (9.16,1.17) -- (9.17,1.16) -- (9.17,1.15) -- (9.17,1.15) -- (9.16,1.14) -- (9.16,1.13) -- (9.15,1.12) -- (9.14,1.12) -- (9.13,1.11) -- (9.11,1.1) -- (9.1,1.1) -- (9.08,1.09) -- (9.07,1.09) -- (9.05,1.09) -- (9.05,1.09) -- (9.03,1.09) -- (9.03,1.09) -- (9.02,1.09) -- (9.02,1.09) -- (9.01,1.09) -- (9.01,1.09) -- (9.01,1.09) -- (9.01,1.09) -- (9.01,1.09) -- (9.01,1.09) -- (9.01,1.08) -- (9.01,1.08) -- (9.01,1.08) -- (9.01,1.08) -- (9.01,1.07) -- (9.01,1.07) -- (9.01,1.07) -- (9.02,1.06) -- (9.02,1.06) -- (9.02,1.05) -- (9.03,1.05) -- (9.04,1.04) -- (9.04,1.03) -- (9.05,1.02) -- (9.06,1.02) -- (9.07,1.01) -- (9.08,1.0) -- (9.1,1.0) -- (9.1,0.99) -- (9.12,0.98) -- (9.13,0.97) -- (9.14,0.97) -- (9.16,0.96) -- (9.16,0.96) -- (9.18,0.96) ;
\draw [stroke] (9.51,1.75) -- (9.51,1.76) -- (9.51,1.76) -- (9.52,1.77) -- (9.52,1.77) -- (9.52,1.78) -- (9.53,1.78) -- (9.53,1.79) -- (9.54,1.79) -- (9.54,1.79) -- (9.55,1.8) -- (9.56,1.81) -- (9.57,1.81) -- (9.58,1.82) -- (9.59,1.82) -- (9.6,1.82) -- (9.62,1.83) -- (9.64,1.84) -- (9.67,1.84) -- (9.7,1.85) -- (9.73,1.85) -- (9.75,1.85) -- (9.77,1.84) -- (9.79,1.84) -- (9.8,1.83) -- (9.8,1.82) -- (9.81,1.81) -- (9.81,1.8) -- (9.81,1.79) -- (9.81,1.78) -- (9.8,1.76) -- (9.79,1.74) -- (9.78,1.71) -- (9.75,1.68) -- (9.72,1.65) -- (9.7,1.62) -- (9.67,1.59) -- (9.64,1.56) -- (9.63,1.53) -- (9.62,1.51) -- (9.61,1.5) -- (9.61,1.49) -- (9.61,1.47) -- (9.61,1.46) -- (9.62,1.45) -- (9.63,1.43) -- (9.64,1.42) -- (9.67,1.4) -- (9.71,1.39) -- (9.76,1.38) -- (9.83,1.38) -- (9.91,1.39) -- (10.0,1.41) ;

		   \end{tikzpicture}
